WearID: Wearable-Assisted Low-Effort Authentication to Voice Assistants using Cross-Domain Speech Similarity

Due to the open nature of voice input, voice assistant (VA) systems (e.g., Google Home and Amazon Alexa) are under a high risk of sensitive information leakage (e.g., personal schedules and shopping accounts). Though the existing VA systems may employ voice features to identify users, they are still vulnerable to various acoustic attacks (e.g., impersonation, replay and hidden command attacks). In this work, we focus on the security issues of the emerging VA systems and aim to protect the users' highly sensitive information from these attacks. Towards this end, we propose a system, WearID, which uses an off-the-shelf wearable device (e.g., a smartwatch or bracelet) as a secure token to verify the user's voice commands to the VA system. In particular, WearID exploits the readily available motion sensors from most wearables to describe the command sound in vibration domain and check the received command sound across two domains (i.e., wearable's motion sensor vs. VA device's microphone) to ensure the sound is from the legitimate user.

==> text_ccs2019/discussion.tex <==
\vspace{-2mm}
\section{Discussion}
\label{sec:discussion}

%For the WiFi-based wearable sensor data logging, we need to talk about the trend of the wearables' that has WiFi module. For the wake word and gesture-based method, we need to say the motion sensor is on for fitness tracking. Such data can also be utilized for detecting the start of voice command without causing much cost.
\vspace{-2mm}
\subsection{Minimum User Participation}
Using a virtual button~\cite{virtualbutton2018} on the wearable devices to use the VA system is quite cumbersome, as the user has to unlock the wearable, find the App (or button), press the button and wait. Moreover, a virtual button cannot verify the command’s sound, which still suffers from the hidden commands and ultrasound attacks. In comparison, our method directly verifies the command sound cross the readily available information from two domains and does not require user interaction with the watch.
\vspace{-2mm}
\subsection{Fall-back Plan}
WearID allows a fall-back plan to improve the user experience. If the user forgets to bring the wearable or fails accessing the VA system for three times, WearID allows the user to use the VA system under the fall-back verification process. In particular, the VA system's cloud server will send a notification message (e.g., voice commands in text) to the user's wearable, from which the user could confirm the voice commands or reset the VA system. If the voice command is not initiated by the legitimate user, the user can use the wearable to reject the voice command. If the user does not bring the wearable, the VA system will ask challenge questions for the user to verify themselves.
\vspace{-2mm}
\subsection{Comparison with Proximity Detection}
Simply detecting proximity between the user and the VA system cannot verify the sound source. Moreover, the existing proximity detection schemes based on Bluetooth or WiFi cannot achieve the short-range proximity detection that the wearable's motion sensor can provide.
%\subsection{Using Motion Sensor Instead of a Second Microphone}
%We choose the motion sensor because of its short and secure response range, a different sensing modality to provide enhanced security, low power consumption, and a wide deployment on wearable devices. All these benefits cannot be provided by a second microphone. Moreover, we do not require much programming or processing on the wearable. The wearable only needs to transmit the motion sensor data, which is already available on most wearable devices.
%Note that if the adversary can issue impersonated commands to the voice assistant’s microphone, it can also do the same to the second microphone, if used.
\vspace{-1mm}
\subsection{Implicit Liveness Detection}
The short response range (e.g., 25cm) of the wearable motion sensor guarantees its received voice sound is from the legitimate user. It is thus not necessary to differentiate human voice from the similar machine sound, because machine sound is hard to be so close to the legitimate user without causing noticed.

%
%As discussed, we allow the user to use smartphone if not having wearable device. If the %user fails three times to access the voice assistant system. It can ask challenge %questions for the user to access and reset the system later.
%
%currently, we only check the similarity between two devices (i.e., voice assistant system and the wearable device). We don't recognize people's voice. As the motion sensors show the possibility of revealing the speaker information. Our system could also work with the existing methods to both detect the co-location of the user with the voice command source and verify the speaker's identity.
%
%how to defend ultrasound attack
%
%%\textbf{How to Address Low-frequency noises. } Air conditioning and people walking.
%
%
%%\textbf{Discuss the Differences of the Recorded Audio Data from the Real Voice Assistant Device and the Smartphone. }
%
%\textbf{identify Confirmation} In this paper, we assume that an adversary can not physically access the voice assistant device or obtain the legitimate the user's wearable. Our system can work with the existing method to identify the user's identity based on motion sensors. So when an adversary has the legitimate the user's wearable, we can still verify the user's identity.



==> text_ccs2019/prototype.tex <==
\section{Prototype}
 
